Portrait Neural Radiance Fields from a Single Image

We present a method for estimating Neural Radiance Fields (NeRF) from a single headshot portrait. While NeRF has demonstrated high-quality view synthesis, it requires multiple images of static scenes and thus impractical for casual captures and moving subjects. In this work, we propose to pretrain the weights of a multilayer perceptron (MLP), which implicitly models the volumetric density and colors, with a meta-learning framework using a light stage portrait dataset. To improve the generalization to unseen faces, we train the MLP in the canonical coordinate space approximated by 3D face morphable models. We quantitatively evaluate the method using controlled captures and demonstrate the generalization to real portrait images, showing favorable results against state-of-the-arts.

==> figure/fig_Xu.tex <==
\begin{figure}[t]
\footnotesize
\includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/4_input_nobg_crop.png}\hfill
\includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/4_r02_Xu_nobg_crop.png}\hfill
\includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/4_r02_ours_crop.png}\hfill

\includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/1_input_nobg_crop.png}\hfill
\includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/1_r02_Xu_nobg_crop.png}\hfill
\includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/1_r02_ours_crop.png}\hfill

% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/5_input_nobg_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/5_r02_Xu_nobg_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/5_r02_ours_crop.png}\hfill

% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/2_input_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/2_r07_Xu_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/2_r07_ours_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/3_input_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/3_r07_Xu_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/3_r07_ours_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/6_input_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/6_r02_Xu_crop.png}\hfill
% \includegraphics[width=0.3315\linewidth]{fig/Xu_comparison/6_r02_ours_crop.png}\hfill


\mpage{0.3}{Input} \hfill
\mpage{0.3}{\cite{Xu-2020-D3P}} \hfill
\mpage{0.3}{Ours} \hfill

\caption{\textbf{Comparison with the Xu \etal \cite{Xu-2020-D3P}}
Using inputs from their paper. Both methods look plausible, while their method is trained on the dataset consisting of 180K individuals, our method requires a much smaller amount of subjects (27 individuals). 
%Note that the Xu \etal \cite{Xu-2020-D3P} focuses on manipulating the \emph{subjects' pose} (i.e., rotating the head only) while our method aims to change the  \emph{camera poses}.
}
\label{fig:Xu_comparison}
\end{figure}

==> figure/fig_reenactment.tex <==
\begin{figure}[h!]
% 
\newlength\figwidthC
\setlength\figwidthC{0.14\linewidth}
% 
\centering%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/314_12_input.png}\\%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/363_12_input.png}\\%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/369_12_input.png}\\%
 \scriptsize Input}%
%
\hfill%
%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/Reenactment/target_16.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/target_16.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/target_16.png}\\%
 \scriptsize Driving view}%
%
\hfill%
%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/Reenactment/314_16_firstorder.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/363_16_firstorder.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/369_16_firstorder.png}\\%
 \scriptsize Siarohin~\etal\cite{siarohin2020first}}%
%
\hfill%
%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/Reenactment/314_16_Bilayer.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/363_16_Bilayer.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/369_16_Bilayer.png}\\%
 \scriptsize Zakharov~\etal\cite{zakharov2020fast}}%
%
\hfill%
%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/Reenactment/314_16_fsv2v.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/363_16_fsv2v.png}\\%
\includegraphics[width=\figwidthC]{fig/Reenactment/369_16_fsv2v.png}\\%
 \scriptsize Wang~\etal\cite{wang2019few}}%
%
\hfill%
%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/314_16_ours.png}\\%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/363_16_ours.png}\\%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/369_16_ours.png}\\%
 \scriptsize Ours}%
\hfill 
%
\parbox[t]{\figwidthC}{\centering%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/314_16_gt.png}\\%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/363_16_gt.png}\\%
\includegraphics[width=\figwidthC]{fig/holodeck_comparison/369_16_gt.png}\\%
 \scriptsize Ground Truth}%
\vspace{1mm}
\caption{\textbf{Comparison to the face reenactment methods on the light stage dataset.} 
The face reenactment methods \cite{siarohin2020first,wang2019few,zakharov2020fast} do not take the camera poses as input, thus a different person with the same ground truth pose to drive the synthesis (second column). The results either lose identity or generate incorrect gaze direction.
}
\label{fig:reenactment}
\end{figure}


==> figure/fig_training_views.tex <==
\begin{figure*}[t]
\footnotesize
%
\newlength\figwidthview
\setlength\figwidthview{0.15\linewidth}
% 
\centering%
\parbox[t]{\figwidthview}{\centering%
\includegraphics[width=\figwidthview]{fig/Training views/000000.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000001.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000002.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000003.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000004.png}\\%
}%
%
\hfill%
%
\parbox[t]{\figwidthview}{\centering%
\includegraphics[width=\figwidthview]{fig/Training views/000005.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000006.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000007.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000008.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000009.png}\\%
}%
%
\hfill%
%
\parbox[t]{\figwidthview}{\centering%
\includegraphics[width=\figwidthview]{fig/Training views/000010.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000011.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000012.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000013.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000014.png}\\%
}%
%
\hfill%
%
\parbox[t]{\figwidthview}{\centering%
\includegraphics[width=\figwidthview]{fig/Training views/000015.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000016.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000017.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000018.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000019.png}\\%
}%
%
\hfill%
%
\parbox[t]{\figwidthview}{\centering%
\includegraphics[width=\figwidthview]{fig/Training views/000020.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000021.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000022.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000023.png}\\%
\includegraphics[width=\figwidthview]{fig/Training views/000024.png}\\%
}%
\vspace{2mm}
\caption{\textbf{Examples of the 5-by-5 training views from a training subject in our light stage dataset.} 
}
\label{fig:training_views}
\end{figure*}


==> table/algorithm.tex <==
\begin{algorithm}[h]
\small
\SetAlgoLined
\SetAlgoNoEnd
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwInOut{Require}{Require}
\Require{$p(\mathcal{T})$: distribution over tasks}
\Require{$\alpha$, $\beta$: step size hyperparameters}
\Require{$N_s$, $N_q$: training iterations}
\Input{Training tasks $\{\mathcal{T}_m\}_0^{K-1}$ from $K$ subjects}
\Output{The pretrained model parameter $\theta_{p,K-1}$ }
Randomly initialize the model $f_\theta$ with $\theta_{p,-1}$ \\
\For{$m = 0 \cdots  K-1$}{
Sample a training task $\mathcal{T}_m \sim p(\mathcal{T})$ \\
$\mathcal{D}_s \gets $ frontal view of $\mathcal{T}_m$ \\
$\mathcal{D}_q \gets $ rest views of $\mathcal{T}_m$ \\
% 
$\theta_m^0 \gets \theta_{p,m-1}$ \\
% 
\For{$t = 0 \cdots (N_s - 1)$}{
Sample a batch $\mathcal{D}_s^t$ from $\mathcal{D}_s$ \\
% 
Evaluate $\nabla_{\theta} \mathcal{L}_{\mathcal{D}_s^t}(f_{\theta_m^t})$ using $\mathcal{D}_s^t$ \\
% 
$\theta_m^{t+1} = \theta_m^t - \alpha \nabla_{\theta} \mathcal{L}_{\mathcal{D}_s^t}(f_{\theta_m^t})$ \\
% 
}
$\theta_m^0 \gets \theta_m^{N_s}$,
% 
$\theta_{p,m}^0 \gets \theta_{p,m-1}$ \\
% 
\For{$t = 0 \cdots (N_q - 1)$}{
Sample a batch $\mathcal{D}_q^t$ from $\mathcal{D}_q$ \\
% 
Evaluate $\nabla_{\theta} \mathcal{L}_{\mathcal{D}_q^t}(f_{\theta_m^t})$ using $\mathcal{D}_q^t$ \\
% 
$\theta_m^{t+1} = \theta_m^t - \beta \nabla_{\theta} \mathcal{L}_{\mathcal{D}_q^t}(f_{\theta_m^t})$ \\
% 
$\theta_{p,m}^{t+1} = \theta_{p,m}^t - \beta \nabla_{\theta} \mathcal{L}_{\mathcal{D}_q^t}(f_{\theta_m^t})$ \\
}
$\theta_{p,m} \gets \theta_{p,m}^{N_q}$ \\
}
\caption{Pretrain NeRF on the light stage dataset. 
% \ckliang{When \emph{done} for the while loop is not stated.}
% \chen{We actually use Adam optimizer.}
}
\label{alg:algorithm}
\end{algorithm}
